Can Deep Learning Predict Risky Retail Investors? A Case Study in Financial Risk Behavior Forecasting

The paper examines the potential of deep learning to support decisions in financial risk management. We develop a deep learning model for predicting whether individual spread traders secure profits from future trades. This task embodies typical modeling challenges faced in risk and behavior forecasting. Conventional machine learning requires data that is representative of the feature-target relationship and relies on the often costly development, maintenance, and revision of handcrafted features. Consequently, modeling highly variable, heterogeneous patterns such as trader behavior is challenging. Deep learning promises a remedy. Learning hierarchical distributed representations of the data in an automatic manner (e.g. risk taking behavior), it uncovers generative features that determine the target (e.g., trader's profitability), avoids manual feature engineering, and is more robust toward change (e.g. dynamic market conditions). The results of employing a deep network for operational risk forecasting confirm the feature learning capability of deep learning, provide guidance on designing a suitable network architecture and demonstrate the superiority of deep learning over machine learning and rule-based benchmarks.

==> outtakes.tex <==

\begin{table}[!htb]
\caption{DNN Performance vs. Benchmarks in terms of P\&L and the AUC} 
\label{tab:cv10}
\begin{tabular}{llllllllllll}
\toprule
 & \multicolumn{11}{c}{Cross-validation folds}                                           \\
 & 1     & 2     & 3     & 4     & 5     & 6     & 7     & 8     & 9     & 10    & mean  \\
\hline
& \multicolumn{11}{l}{Average P\&L per trader in GBP} \\
\hline
no hedging & 2268  & 2130  & 1601  & 2122  & 2230  & 2536  & 1785  & 1938  & 1870  & 2306  & 2079 \\

DNN & 2245  & 2906  & 3490  & 2863  & 2245  & 3536  & 2679  & 3536  & 3014  & 2792  & 2931  \\
Logit & 3021  & 2281  & 2901  & 2707  & 3413  & 2643  & 2443  & 2358  & 2452  & 2679  & 2690  \\
ANN  & 2619  & 2624  & 2207  & 2614  & 3002  & 2515  & 2594  & 2503  & 2691  & 2920  & 2629  \\
RF & 2745  & 2539  & 2255  & 2559  & 2574  & 3198  & 2624  & 2295  & 2578  & 2451  & 2582  \\
AdaBoost & 2402  & 2756  & 1869  & 1857  & 2435  & 2956  & 2215  & 2482  & 2672  & 2741  & 2439  \\
SVM & 1511  & 2656  & 1382  & 1278  & 1140  & 1796  & 835  & 3149  & 312  & 2402  & 1646  \\
\hline
& \multicolumn{11}{l}{Area Under Receiver-Operating Characteristics Curve (AUC)}        \\
\hline
DNN & 0.816 & 0.806 & 0.809 & 0.802 & 0.826 & 0.804 & 0.842 & 0.816 & 0.782 & 0.832 & 0.814 \\
ANN & 0.633 & 0.643 & 0.645 & 0.638 & 0.625 & 0.645 & 0.640 & 0.645 & 0.618 & 0.616 & 0.635 \\
Logit & 0.708 & 0.698 & 0.716 & 0.699 & 0.690 & 0.704 & 0.735 & 0.692 & 0.708 & 0.701 & 0.705 \\
RF & 0.714 & 0.734 & 0.726 & 0.728 & 0.736 & 0.721 & 0.710 & 0.717 & 0.684 & 0.730 & 0.720 \\
AdaBoost 
    & 0.647 & 0.631 & 0.637 & 0.618 & 0.648 & 0.656 & 0.635 & 0.650 & 0.625 & 0.632 & 0.638 \\
SVM
    & 0,688 & 0,887 & 0,692 & 0,691 & 0,794 & 0,664 & 0,695 & 0,586 & 0,625 & 0,592&0,690 \\
\bottomrule \bottomrule 
\end{tabular}
\end{table}



\begin{table}[!htb]
\caption{Average P\&L per trader in GBP of the DNN-Based and Rule-Based Hedging Strategies} 
\label{tab:hedging_heuristics}
\begin{tabular}{llllllllllll}
\toprule
 & \multicolumn{11}{c}{Cross-validation folds}  \\
 & 1        & 2              & 3              & 4              & 5              & 6              & 7              & 8              & 9              & 10             & mean                           \\
\hline
no hedge & 2.268          & 2.130          & 1.601          & 2.122          & 2.230          & 2.536          & 1.785          & 1.938          & 1.870          & 2.306          & 2.079          \\
\hline
DNN      & \textbf{2.245} & \textbf{2.906} & \textbf{3.490} & \textbf{2.863} & \textbf{2.245} & \textbf{3.536} & \textbf{2.679} & \textbf{3.536} & \textbf{3.014} & \textbf{2.792} & \textbf{2.931} \\
STX      & 2.014          & 2.229          & 2.155          & 2.238          & 1.878          & 1.913          & 1.872          & 2.190          & 2.937          & 1.811          & 2.124          \\
custom 1 & 1.534          & 1.549          & 1.236          & 1.550          & 1.417          & 1.488          & 1.392          & 1.618          & 1.986          & 1.341          & 1.511          \\
custom 2 & 1.969          & 1.831          & 1.486          & 1.440          & 2.299          & 1.724          & 2.076          & 1.594          & 1.594          & 2.046          & 1.806          \\
custom 3 & 1.736          & 1.825          & 1.579          & 1.965          & 1.865          & 1.937          & 2.000          & 1.785          & 2.402          & 1.750          & 1.884          \\
ensemble & 1.869          & 1.950          & 1.530          & 2.151          & 1.897          & 1.852          & 1.784          & 1.656          & 2.480          & 1.693          & 1.886         \\
\hline
%decision stump	& 2.010 & 	1.434 	& 2.459 	& 2.272 &	2.234 &	2.309 &	2.083 &	2.048 &	2.166 & 	2.119 &	2.113 \\
ctree &	2.163 &	1.544 &	2.799 &	2.154 &	2.089 &	2.299 &	1.972 &	2.051 &	2.215 & 1.974 &	2.126 \\
\bottomrule \bottomrule 
\end{tabular}
%\begin{tablenotes}
%\item\emph{Notes:} We 
%\end{tablenotes}
\end{table}
